Enhancement of Retinal Fundus Images via Pixel Color Amplification

We propose a pixel color amplification theory and family of enhancement methods to facilitate segmentation tasks on retinal images. Our novel re-interpretation of the image distortion model underlying dehazing theory shows how three existing priors commonly used by the dehazing community and a novel fourth prior are related. We utilize the theory to develop a family of enhancement methods for retinal images, including novel methods for whole image brightening and darkening. We show a novel derivation of the Unsharp Masking algorithm. We evaluate the enhancement methods as a pre-processing step to a challenging multi-task segmentation problem and show large increases in performance on all tasks, with Dice score increases over a no-enhancement baseline by as much as 0.491. We provide evidence that our enhancement preprocessing is useful for unbalanced and difficult data. We show that the enhancements can perform class balancing by composing them together.

==> fig-rite_segmentation.tex <==
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/rite_segmentation.png}
  % \includegraphics[width=0.32\linewidth]{name.ext}
  % \includegraphics[width=0.32\linewidth]{name.ext}
  \caption{\textbf{Vessel Segmentation on RITE}.  White pixels show agreement.  Red pixels show sC+sX model predicted positive.  Cyan pixels show the ground truth (left) or baseline identity (right) predicted positive.  Using our enhancement results in a better vessel tree.}
\label{fig:rite_segmentation}
\end{figure}


==> fig-segmentation_maps.tex <==
\begin{figure}[htpb]
  \centering
  \begin{subfigure}[]{\textwidth}
  \begin{center}
    % \includegraphics[width=0.8\linewidth]{segment_rite.png}
  \end{center}
  \caption{RITE}
  \label{fig:segment_rite}
  \end{subfigure}
  \begin{subfigure}[]{\textwidth}
  \begin{center}
    % \includegraphics[width=0.8\linewidth]{segment_idrid.png}
  \end{center}
  \caption{}
  \label{fig:segment_idrid}
  \end{subfigure}
  % \caption{Name}
  % TODO captions
  \label{fig:segmentation_maps}
  \caption{Segmentation maps for RITE and IDRID.  Predicted segmentation is green, ground truth is magenta, and overlap is white. }
\end{figure}


==> figures/qualdr_mcc_top_models.tex <==
\begin{tabular}{|lll}
\toprule
     Task & Method &   Dice (delta) \\
\midrule
 arteries &      A &  0.558 (0.083) \\
  overlap &      A &  0.194 (0.067) \\
    veins &      A &  0.638 (0.044) \\
  vessels &      A &  0.799 (0.037) \\
\bottomrule
\end{tabular}


==> figures/qualdr_top_models.tex <==
\begin{tabular}{|lll}
\toprule
   &   &    MCC (delta) \\
\textbf{Task} & \textbf{Method} &                \\
\midrule
\multirow{2}{*}{\textbf{DR}} & \textbf{avg3:A+B+X} &  0.549 (0.071) \\
   & \textbf{avg2:sC+sX} &  0.544 (0.066) \\
\cline{1-3}
\multirow{2}{*}{\textbf{MD}} & \textbf{avg5:sA+sB+sC+sW+sX} &  0.654 (0.088) \\
   & \textbf{avg4:A+B+C+X} &  0.651 (0.085) \\
\cline{1-3}
\multirow{2}{*}{\textbf{PC}} & \textbf{avg3:A+B+X} &  0.663 (0.225) \\
   & \textbf{B} &  0.655 (0.217) \\
\bottomrule
\end{tabular}


==> figures/rite_top_models.tex <==
\begin{tabular}{|lll}
\toprule
        &          &   Dice (delta) \\
\textbf{Task} & \textbf{Method} &                \\
\midrule
\multirow{2}{*}{\textbf{Arteries}} & \textbf{avg4:sA+sB+sC+sX} &  0.602 (0.127) \\
        & \textbf{avg2:C+X} &  0.591 (0.116) \\
\cline{1-3}
\multirow{2}{*}{\textbf{Overlap}} & \textbf{avg2:sC+sX} &  0.336 (0.209) \\
        & \textbf{avg3:sA+sC+sX} &  0.334 (0.207) \\
\cline{1-3}
\multirow{2}{*}{\textbf{Veins}} & \textbf{avg2:sC+sX} &  0.677 (0.083) \\
        & \textbf{avg3:A+C+X} &  0.674 (0.080) \\
\cline{1-3}
\multirow{2}{*}{\textbf{Vessels}} & \textbf{avg2:sC+sX} &  0.818 (0.056) \\
        & \textbf{avg2:C+X} &  0.815 (0.054) \\
\bottomrule
\end{tabular}


==> figures/top15-separability.tex <==
\begin{tabular}{lr}
\toprule
              Method &  Separability score \\
\midrule
                   A &            0.419957 \\
            avg2:A+X &            0.385313 \\
            avg2:A+B &            0.382486 \\
          avg2:sA+sB &            0.380456 \\
          avg3:A+B+X &            0.380307 \\
          avg2:sA+sX &            0.379259 \\
                   B &            0.367973 \\
       avg3:sA+sB+sX &            0.361331 \\
            avg2:B+X &            0.340273 \\
                   X &            0.334064 \\
        avg4:A+B+C+X &            0.333409 \\
          avg2:sB+sX &            0.326207 \\
          avg3:B+C+X &            0.317462 \\
      avg5:A+B+C+W+X &            0.309622 \\
 avg5:sA+sB+sC+sW+sX &            0.309406 \\
            identity &            0.304329 \\
\bottomrule
\end{tabular}


==> table-top_qualdr.tex <==
\begin{figure}
  \centering
  \begin{minipage}{0.49\textwidth}
  \centering
  \captionsetup{type=table}
  \scriptsize
  \caption{QualDR: Top Models}
  \input{figures/qualdr_top_models.tex}
  \label{table:qualdr_top}
\end{minipage}%
\begin{minipage}{0.49\textwidth}
  \centering
    \begin{center}
      \includegraphics[width=\linewidth]{figures/correlation_mcc_qualdr_test.png}
    \end{center}
    \label{fig:correlation_mcc_qualdr_test}
\end{minipage}
    \caption{QualDR evaluation.  Left: Best performing models.  Right: Correlation between Separability score (IDRiD Train) and MCC (QualDR Test).  Legend shows Pearson correlation and p-value.}
\end{figure}


==> table_qualdr.tex <==
% % version 1
% \begin{tabular}{lllllll}
% \toprule
% {} & \multicolumn{2}{l}{DR} & \multicolumn{2}{l}{MD} & \multicolumn{2}{l}{PC} \\
% {} &       Train &        Test &       Train &        Test &       Train &        Test \\
% \midrule
% -1.0 &   54 (6.5\%) &   30 (8.4\%) &  227(27.4\%) &  101(28.4\%) &   73 (8.8\%) &  37 (10.4\%) \\
%  0.0 &  315(38.0\%) &  119(33.4\%) &  500(60.3\%) &  209(58.7\%) &  735(88.7\%) &  306(86.0\%) \\
%  1.0 &  158(19.1\%) &  63 (17.7\%) &  102(12.3\%) &  46 (12.9\%) &   11 (1.3\%) &   4  (1.1\%) \\
%  2.0 &  187(22.6\%) &  89 (25.0\%) &         --- &         --- &   10 (1.2\%) &   9  (2.5\%) \\
%  3.0 &   42 (5.1\%) &   21 (5.9\%) &         --- &         --- &         --- &         --- \\
%  4.0 &   73 (8.8\%) &   34 (9.6\%) &         --- &         --- &         --- &         --- \\
% \bottomrule
% \end{tabular}
% version 2
\begin{tabular}{l|rr|rr|rr}
\toprule
  {} & \multicolumn{2}{l}{\textbf{DR}} & \multicolumn{2}{l}{\textbf{MD}} & \multicolumn{2}{l}{\textbf{PC}} \\
{\scriptsize Grade} &\scriptsize  Train &\scriptsize  Test &\scriptsize  Train &\scriptsize  Test &\scriptsize  Train &\scriptsize  Test \\
\midrule
-1.0 &    54 &   30 &   227 &  101 &    73 &   37 \\
 0.0 &   315 &  119 &   500 &  209 &   735 &  306 \\
 1.0 &   158 &   63 &   102 &   46 &    11 &    4 \\
 2.0 &   187 &   89 &   --- &  --- &    10 &    9 \\
 3.0 &    42 &   21 &   --- &  --- &   --- &  --- \\
 4.0 &    73 &   34 &   --- &  --- &   --- &  --- \\
\bottomrule
\end{tabular}


==> tables_top_scores.tex <==
\begin{figure}
  \centering
  \begin{minipage}[t]{0.49\textwidth}
  \centering
  \captionsetup{type=table}
  % \caption{Top $S_\text{KS}$ scores (IDRiD Train set)}
  % \small
  % \input{figures/top15-separability.tex}
  % \label{table:separability}
  \scriptsize
  \caption{IDRiD: Top Models}
  \input{figures/idrid_top_models.tex}
  \label{table:idrid_top}
  \caption{QualDR: Top Models}
  \input{figures/qualdr_top_models.tex}
  \label{table:qualdr_top}
\end{minipage}%
\begin{minipage}[t]{0.49\textwidth}
  \captionsetup{type=table}
  \centering
  \caption{RITE: Top Models}
  \scriptsize
  \input{figures/rite_top_models.tex}
  \label{table:rite_top}
  \begin{center}
    \includegraphics[width=.98\linewidth,right]{figures/correlation_mcc_qualdr_test.png}
  \end{center}
  \label{fig:correlation_mcc_qualdr_test}
\end{minipage}
\caption{\textbf{Performance Evaluation}}%: The tables show the test set Dice or MCC value of the top two best performing models for each dataset and task. The plot shows a correlation between Separability score (IDRiD Train) and MCC (QualDR Test), and legend shows Pearson correlation (R) and p-value.}
\end{figure}

